Win-Fail Action Recognition

Current video/action understanding systems have demonstrated impressive performance on large recognition tasks. However, they might be limiting themselves to learning to recognize spatiotemporal patterns, rather than attempting to thoroughly understand the actions. To spur progress in the direction of a truer, deeper understanding of videos, we introduce the task of win-fail action recognition -- differentiating between successful and failed attempts at various activities. We introduce a first of its kind paired win-fail action understanding dataset with samples from the following domains: "General Stunts," "Internet Wins-Fails," "Trick Shots," and "Party Games." Unlike existing action recognition datasets, intra-class variation is high making the task challenging, yet feasible. We systematically analyze the characteristics of the win-fail task/dataset with prototypical action recognition networks and a novel video retrieval task. While current action recognition methods work well on our task/dataset, they still leave a large gap to achieve high performance. We hope to motivate more work towards the true understanding of actions/videos. Dataset will be available from https://github.com/ParitoshParmar/Win-Fail-Action-Recognition.

==> Sections/Models.tex <==
\section{Models}
\label{sec:Models}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figs/model_indi_pairwise_cropped.pdf}
    \caption{Models: Individual (a) and Pairwise (b). 00 and 11 in pairwise are equivalent to 0 and 1 in individual.}
    \label{fig:models_indi_pair}
\end{figure}
We use a CNN ($G$) to compute spatial features, followed by a temporal model ($F$) to compute temporal relationships from spatial features from $G$. In particular, we consider temporal order agnostic (\textit{averaging} of activations from $G$) and temporal order respecting (LSTM \cite{lstm} and TRN \cite{trn}) as our temporal models. 

We use cross-entropy loss, $\mathcal{L}$ as the objective function to train the networks. Let $x_{i}$ and $y_{i}$ be the predicted and ground-truth labels, then,

\begin{equation}
\label{eq:xentropy_loss}
 \mathcal{L} = -\frac{1}{N} \sum_{i=1}^{N} y_{i}logx_{i}
\end{equation}

We experiment with the following two approaches for win-fail action recognition task.
 
\paragraph{Individual/standalone analysis}
Individual analysis is identical to any typical image/action classification, where we process the images/video-clip through network, and it predicts the class (win or fail in our case). Model is illustrated in Fig. \ref{fig:models_indi_pair} (a).

\begin{equation}
 x_{i} = H(F(G(V))) 
\end{equation}
 
where, $V$ is input video frames in the case $G$ is a 2D-CNN, or it is video clips if $G$ is a 3D-CNN; and $H$ represents a linear layer. This is a binary classification problem: $x_{i}, y_{i} \in \{0, 1\}$.

	
\paragraph{Pairwise analysis}

[TODO: mention that paired/pairwise nature of the data is leveraged]

In pairwise analysis, we use a siamese setup, as shown in Fig. \ref{fig:models_indi_pair} (b). Let $V_{a}$ and $V_{b}$ represent two input videos, then,

\begin{equation}
x_{i} = H(C(F(G(V_{a})), F(G(V_{b}))))
\end{equation}

where, $C$ is the concatenation operation. We allow $V_{a} = V_{b}$ to incorporate individual/standalone analysis of samples. We see pairwise loss as an aid to the learning process. In all, pairwise analysis would be a four-way classification problem: $x_{i}, y_{i} \in \{00, 01, 10, 11\}$.


==> Tables/tab_incomplete_seq.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\small
\centering
\begin{tabular}{@{}lc@{}}
\toprule
\textbf{Observed   sequence} & \textbf{Accuracy} \\ \midrule
Full                         & 74.78             \\ \midrule
First $1/4$                      & 25.13             \\
First $1/2$                      & 35.62             \\
First $3/4$                      & 48.60             \\ \midrule
Last $1/4$                       & 23.47             \\
Last $1/2$                       & 28.93             \\
Last $3/4$                       & 52.58             \\ \bottomrule
\end{tabular}
\vspace{0.2cm}
\caption{\textbf{Partial observations.}}
\label{tab:incomplete_seq}
\end{table}

==> Tables/tab_reverse_seq.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\small
\begin{tabular}{lcccc}
\toprule
Model      & {\color[HTML]{9B9B9B} \begin{tabular}[c]{@{}c@{}}Acc.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}$\Delta1$\\ ($\uparrow$ is better)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\Delta2$\\ ($\downarrow$ is better)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$|\Delta2:\Delta1|$\\ ($\downarrow$ is better)\end{tabular} \\ 
\midrule
BL-1 & {\color[HTML]{9B9B9B} 48.79}                                                           & -1.39                                                                & -3.15                                                               & 2.26                                                                        \\ 
BL-2 & {\color[HTML]{9B9B9B} 45.28}                                                           & 6.47                                                                 & -6.12                                                               & 0.94                                                                        \\ 
BL-3 & {\color[HTML]{9B9B9B} 61.45}                                                           & 6.47                                                                 & -35.14                                                              & 5.43                                                                        \\ 
Ours       & {\color[HTML]{9B9B9B} 74.78}                                                           & \textbf{69.41}                                                       & -10.49                                                              & \textbf{0.15}                                                               \\ \bottomrule
\end{tabular}
\caption{\textbf{Reversing sequences.}}
\label{tab:reversed_seq}
\end{table}

==> Tables/tab_scrambling.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{@{}lc@{}}
\toprule
\textbf{Shuffle type} & \textbf{Accuracy} \\ \midrule
None                     & 74.78             \\
First $1/3$               & 74.16             \\
Middle $1/3$              & 74.26             \\
Last $1/3$                & 72.42             \\
Full                     & 61.19             \\ \bottomrule
\end{tabular}
\vspace{0.2cm}
\caption{\textbf{Effect of shuffling.}}
\label{tab:scrambling}
\end{table}

==> Tables/tab_trn_vs_lstm.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\small
\centering
\begin{tabular}{lcc}
\toprule
\textbf{Training}    & \textbf{LSTM} & \textbf{TRN}   \\ \midrule
Only temporal module & 68.88         & \textbf{71.24} \\
End-to-End           & 74.78         & \textbf{75.74} \\ \bottomrule
\end{tabular}
%
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{00} & \textbf{01} & \textbf{10} & \textbf{11} \\ \midrule
79.20       & 70.28       & 70.28       & 79.37       \\ \bottomrule
\end{tabular}
%
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{00} & \textbf{01} & \textbf{10} & \textbf{11} \\ \midrule
79.90       & 73.60       & 72.40       & 77.10       \\ \bottomrule
\end{tabular}
%
\caption{\textbf{LSTM vs. TRN.}}
\label{tab:res_lstm_trn}
\end{table}
